Asymmetric Certified Robustness via Feature-Convex Neural Networks

Recent works have introduced input-convex neural networks (ICNNs) as learning models with advantageous training, inference, and generalization properties linked to their convex structure. In this paper, we propose a novel feature-convex neural network architecture as the composition of an ICNN with a Lipschitz feature map in order to achieve adversarial robustness. We consider the asymmetric binary classification setting with one "sensitive" class, and for this class we prove deterministic, closed-form, and easily-computable certified robust radii for arbitrary $\ell_p$-norms. We theoretically justify the use of these models by characterizing their decision region geometry, extending the universal approximation theorem for ICNN regression to the classification setting, and proving a lower bound on the probability that such models perfectly fit even unstructured uniformly distributed data in sufficiently high dimensions. Experiments on Malimg malware classification and subsets of MNIST, Fashion-MNIST, and CIFAR-10 datasets show that feature-convex classifiers attain state-of-the-art certified $\ell_1$-radii as well as substantial $\ell_2$- and $\ell_{\infty}$-radii while being far more computationally efficient than any competitive baseline.

==> extra.tex <==
We now characterize the robustness of $\f\in\F$ around inputs associated to \cns. In this case, we cannot provide norm-ball guarantees by appealing to first-order overestimations of the confidence $\g$, since this is not a concave function in general. To overcome this hurdle, we may appeal to a quadratic overestimation under the assumption that $\g$ is $\beta$-smooth.

\begin{definition}
	\label{def: beta-smooth}
	Let $\beta\in\R$ and let $\|\cdot\|,\|\cdot\|'$ be norms on $\Rd$. A function $g \colon \Rd \to \R$ is called \emph{$\beta$-smooth (with respect to the norms $(\|\cdot\|,\|\cdot\|')$)} if it is continuously differentiable and satisfies $\| \nabla g (x) - \nabla g (y) \| \le \beta \|x-y\|'$ for all $x,y\in\Rd$.
\end{definition}

\begin{remark}
	A twice-differentiable function $g \colon \Rd \to \R$ is $\beta$-smooth with respect to $(\|\cdot\|_2,\|\cdot\|_2)$ if and only if the eigenvalues of the Hessian matrix $\nabla^2 g(x)$ are less than or equal to $\beta$ in absolute value for all $x\in\Rd$ \citep[Section 3.2]{bubeck2015convex}.
\end{remark}

\begin{theoremrep}
	\label{thm: false_positive_robustness}

	Let $\f\in\F$ and let $x\in \f^{-1}(\{2\}) = \{y\in\Rd : \f(y) = 2\}$. If $\g$ is $\beta$-smooth with respect to $(\|\cdot\|_*,\|\cdot\|)$, then it holds that $\f(x+\delta) = 2$ for all $\delta\in\Rd$ such that
	\begin{equation*}
		\|\delta\| \le r_2(x) \coloneqq \frac{\left(\|\nabla \g(x)\|_*^2 - 2\beta \g(x)\right)^{1 / 2} - \|\nabla \g(x)\|_*}{\beta}.
	\end{equation*}
\end{theoremrep}

\begin{proof}
	Suppose that $\g$ is $\beta$-smooth with respect to $(\|\cdot\|_*,\|\cdot\|)$, and let $\delta\in\Rd$ be such that $\|\delta\| \le r_2(x)$. Then by Lemma 3.4 in \citet{bubeck2015convex}, it holds that
	\begin{equation*}
		\g(x+\delta) \le \g(x) + \nabla \g(x)^\top \delta + \frac{\beta}{2}\|\delta\|^2.
	\end{equation*}
	Thus, by the Cauchy-Schwarz inequality for dual norms, we find the following quadratic (in $r_2(x)$) overestimation of $\g$ around $x$:
	\begin{align*}
		\g(x+\delta) &\le \g(x) + \| \nabla \g(x)\|_* \|\delta\| + \frac{\beta}{2}\|\delta\|^2 \\
				    &\le \g(x) + \|\nabla \g(x)\|_* r_2(x) + \frac{\beta}{2} r_2(x)^2.
	\end{align*}
	By Definition of $r_2(x)$, this implies that $\g(x+\delta) \le 0$, and hence $\f(x+\delta) = 2$.
\end{proof}

\begin{comment}% Old proof (overly complicated, restricted to \ell_2)
\begin{proof}
	Suppose that $g_1-g_2$ is $\beta$-smooth with respect to $\|\cdot\|_2$, and let $\delta\in\Rd$ be such that $\|\delta\|_2 \le r_2(x)$. Then by Lemma 3.4 in \citet{bubeck2015convex}, it holds that
	\begin{equation*}
		(g_1-g_2)(x+\delta) \le (g_1-g_2)(x) + \nabla (g_1-g_2)(x)^\top \delta + \frac{\beta}{2}\|\delta\|_2^2.
	\end{equation*}
	Thus, we obtain the following quadratic underestimation of $g_2-g_1$ around $x$:
	\begin{equation*}
		(g_2-g_1)(x+\delta) \ge Q(\delta) \coloneqq -\delta^\top \left(\frac{\beta}{2} I_d\right) \delta +  \nabla (g_2-g_1)(x)^\top\delta + (g_2-g_1)(x).
	\end{equation*}
	Hence,
	\begin{equation}
		(g_2-g_1)(x+\delta) \ge \inf\{Q(\epsilon) : \|\epsilon\|_2 \le r_2(x), ~ \epsilon\in\Rd\} = \inf\{ Q(r_2(x) \epsilon) : \epsilon^\top\epsilon \le 1, ~ \epsilon\in\Rd\}. \label{eq: quadratic_underestimation}
	\end{equation}
	We now proceed with solving the above minimization. Denote the objective function by $P \colon \epsilon \mapsto Q(r_2(x)\epsilon)$ and the constraint function by $H \colon \epsilon\mapsto \epsilon^\top\epsilon - 1$. Note that the optimization problem is nonconvex, as we are minimizing a concave function.

	First, notice that every nonzero feasible point is a regular point, since the gradient of the constraint function $\nabla H(\epsilon) = 2\epsilon$ forms a linearly independent set if and only if $\epsilon \ne 0$. Thus, every nonzero local minimizer must satisfy the Karush-Kuhn-Tucker (KKT) conditions \citep[Proposition 4.3.1]{bertsekas2016nonlinear}. Furthermore, since the objective function is continuous and the feasible set is compact, the infimum is attained and hence all global minimizers must either satisfy the KKT conditions or be $\epsilon^\star = 0$. Thus, suppose that a nonzero local minimizer exists, and denote it by $\epsilon^\star$. Then there exists a unique scalar $\mu^\star \in\R$ such that
	\begin{align}
		&\nabla_\epsilon \left. \left( P(\epsilon) + \mu H(\epsilon) \right) \right|_{(\epsilon,\mu)=(\epsilon^\star,\mu^\star)} = 0, \tag{Lagrangian stationarity} \\
		&\mu^\star H(\epsilon^\star) = 0, \tag{complementary slackness} \\
		&\mu^\star \ge 0, \tag{dual feasibility} \\
		&H(\epsilon^\star) \le 0. \tag{primal feasibility}
	\end{align}
	
	Suppose first that $\mu^\star > 0$. Then $H(\epsilon^\star) = 0$, meaning $\epsilon^\star$ is on the boundary of the unit ball in $\Rd$. Lagrangian stationarity then yields that
	\begin{equation*}
		(2\mu^\star-\beta r_2(x)^2)\epsilon^\star + r_2(x) \nabla (g_2-g_1)(x) = 0.
	\end{equation*}
	If $r_2(x)=0$ or $\nabla g_2(x)=\nabla g_1(x)$, then either $\mu^\star = \frac{\beta r_2(x)^2}{2}$ or $\epsilon^\star = 0$, the latter of which result contradicts the fact that $\epsilon^\star$ is on the boundary of the unit ball. Hence, in this case, it must be that $\mu^\star = \frac{\beta r_2(x)^2}{2}$, and the KKT conditions are satisfied for all $\epsilon^\star\in\Rd$ such that $\|\epsilon^\star\|_2=1$. The minimum objective function value amongst such KKT pairs is
	\begin{align*}
		\inf\{P(\epsilon^\star) : \|\epsilon^\star\|_2 = 1, ~ \epsilon^\star \in \Rd\} &= (g_2-g_1)(x) - \frac{\beta r_2(x)^2}{2} \\
											       &\quad + r_2(x)\inf\{\nabla (g_2-g_1)(x)^\top \epsilon^\star : \|\epsilon^\star\|_2 = 1, ~ \epsilon^\star \in\Rd\} \\
											       &= (g_2-g_1)(x) - \frac{\beta r_2(x)^2}{2} - r_2(x)\|\nabla (g_2-g_1)(x)\|_2 \\
											       &= (g_2-g_1)(x) - \frac{\beta r_2(x)^2}{2}.
	\end{align*}

	On the other hand, if $r_2(x) \nabla (g_2-g_1)(x) \ne 0$, then it must be that $2\mu^\star - \beta r_2(x)^2 \ne 0$ and hence
	\begin{equation*}
		\epsilon^\star = \frac{r_2(x) \nabla (g_2-g_1)(x)}{\beta r_2(x)^2 - 2\mu^\star}.
	\end{equation*}
	In this case, primal feasibility requires that
	\begin{equation*}
		\|\epsilon^\star\|_2 = \frac{r_2(x) \|\nabla (g_2-g_1)(x)\|_2}{|\beta r_2(x)^2 - 2\mu^\star|} = 1.
	\end{equation*}
	which in turn implies that
	\begin{equation*}
		\mu^\star = \frac{r_2(x) (\beta r_2(x) + \|\nabla (g_2-g_1)(x)\|_2)}{2},
	\end{equation*}
	or
	\begin{equation*}
		\mu^\star = \frac{r_2(x)(\beta r_2(x) - \|\nabla (g_2-g_1)(x)\|_2)}{2},
	\end{equation*}
	the latter value of which is only permissible if $\beta \ge \frac{\|\nabla (g_2-g_1)(x)\|_2}{r_2(x)}$, since $r_2(x)>0$. The corresponding primal points are
	\begin{equation*}
		\epsilon^\star = -\frac{\nabla (g_2-g_1)(x)}{\|\nabla (g_2-g_1)(x)\|_2}
	\end{equation*}
	and
	\begin{equation*}
		\epsilon^\star = \frac{\nabla (g_2-g_1)(x)}{\|\nabla (g_2-g_1)(x)\|_2},
	\end{equation*}
	respectively. The objective function value at these KKT pairs are
	\begin{equation*}
		P(\epsilon^\star) = (g_2-g_1)(x) - \frac{\beta r_2(x)^2}{2} - r_2(x) \|\nabla (g_2-g_1)(x)\|_2
	\end{equation*}
	and
	\begin{equation*}
		P(\epsilon^\star) = (g_2-g_1)(x) - \frac{\beta r_2(x)^2}{2} + r_2(x) \|\nabla (g_2-g_1)(x)\|_2,
	\end{equation*}
	respectively. At this point, we have computed all KKT pairs with $\mu^\star>0$ and their associated objective function values.

	Next, suppose that $\mu^\star = 0$. Then, in general, $\epsilon^\star$ may be in the interior of the unit ball. Lagrangian stationarity yields that
	\begin{equation*}
		\beta r_2(x)^2 \epsilon^\star = r_2(x) \nabla (g_2-g_1)(x).
	\end{equation*}
	If $r_2(x) = 0$ or $\nabla g_2(x) = \nabla g_1(x)$, then either $\beta r_2(x)^2 = 0$ or $\epsilon^\star = 0$, the latter of which result contradicts the supposition that $\epsilon^\star$ is nonzero. Hence, in this case, it must be that $\beta r_2(x)^2 = 0$, and the KKT conditions are satisfied for all $\epsilon^\star\in\Rd$ such that $\|\epsilon^\star\|_2 \le 1$. The minimum objective function value amongst such KKT pairs is computed as in the $\mu^\star>0$ case to be
	\begin{equation*}
		\inf\{P(\epsilon^\star) : \|\epsilon^\star\|_2 \le 1, ~ \epsilon^\star\in\Rd\} = (g_2-g_1)(x) - \frac{\beta r_2(x)^2}{2}.
	\end{equation*}

	On the other hand, if $r_2(x) \nabla (g_2-g_1)(x) \ne 0$, then it must be that $\beta r_2(x)^2 \ne 0$ and hence
	\begin{equation*}
		\epsilon^\star = \frac{\nabla (g_2-g_1)(x)}{\beta r_2(x)}.
	\end{equation*}
	In this case, primal feasibility requires that
	\begin{equation*}
		\|\epsilon^\star\|_2 = \frac{\|\nabla (g_2-g_1)(x)\|_2}{\beta r_2(x)} \le 1.
	\end{equation*}
	The objective function value at this KKT pair is
	\begin{equation*}
		P(\epsilon^\star) = (g_2-g_1)(x) - \frac{\|\nabla (g_2-g_1)(x)\|_2^2}{2\beta}.
	\end{equation*}
	At this point, we have computed all KKT pairs with $\mu^\star=0$ and their associated objective function values.

	We now conclude with solving the optimization problem of interest. If $r_2(x)=0$ or $\nabla g_2(x)=\nabla g_1(x)$, the above analysis shows that the minimum objective value amongst all KKT pairs is
	\begin{align*}
		P(\epsilon^\star) &= (g_2-g_1)(x) - \frac{\beta r_2(x)^2}{2}\\
				  &\le (g_2-g_1)(x) \\
				  &= P(0).
	\end{align*}
	Hence, if $r_2(x) = 0$ or $\nabla g_2(x) = \nabla g_1(x)$, we conclude that the optimization yields
	\begin{align*}
		\inf\{P(\epsilon) : H(\epsilon) \le 0, ~ \epsilon\in\Rd\} &= (g_2-g_1)(x) - \frac{\beta r_2(x)^2}{2} \\
	&= (g_2-g_1)(x) - \frac{\beta r_2(x)^2}{2} - r_2(x)\|\nabla (g_2-g_1)(x)\|_2.
	\end{align*}
	
	If $r_2(x)\ne 0$ and $\nabla g_2(x) \ne \nabla g_1(x)$ and $\beta \ge \frac{\| \nabla (g_2-g_1)(x)\|_2}{r_2(x)}$, the above analysis shows that the minimum objective value amongst all KKT pairs is
	\begin{align*}
		P(\epsilon^\star) &= (g_2-g_1)(x) - \frac{\beta r_2(x)^2}{2} - r_2(x)\|\nabla (g_2-g_1)(x)\|_2 \\
				  &\le (g_2-g_1)(x) \\
				  &= P(0).
	\end{align*}
	Hence, if $r_2(x)\ne 0$ and $\nabla g_2(x)\ne\nabla g_1(x)$ and $\beta \ge \frac{\|\nabla (g_2-g_1)(x)\|_2}{r_2(x)}$, we conclude that the optimization yields
	\begin{equation*}
		\inf\{P(\epsilon) : H(\epsilon) \le 0, ~ \epsilon\in\Rd\} = (g_2-g_1)(x) - \frac{\beta r_2(x)^2}{2} - r_2(x)\|\nabla (g_2-g_1)(x)\|_2.
	\end{equation*}
	
	If $r_2(x)\ne 0$ and $\nabla g_2(x)\ne \nabla g_1(x)$ and $\beta < \frac{\|\nabla (g_2-g_1)(x)\|_2}{r_2(x)}$, the above analysis shows that the minimum objective value amongst all KKT pairs is
	\begin{align*}
		P(\epsilon^\star) &= (g_2-g_1)(x) - \frac{\beta r_2(x)^2}{2} - r_2(x)\|\nabla (g_2-g_1)(x)\|_2 \\
				  &\le (g_2-g_1)(x) \\
				  &= P(0).
	\end{align*}
	Hence, if $r_2(x)\ne 0$ and $\nabla g_2(x)\ne\nabla g_1(x)$ and $\beta < \frac{\|\nabla (g_2-g_1)(x)\|_2}{r_2(x)}$, we conclude that the optimization yields
	\begin{equation*}
		\inf\{P(\epsilon) : H(\epsilon) \le 0, ~ \epsilon\in\Rd\} = (g_2-g_1)(x) - \frac{\beta r_2(x)^2}{2} - r_2(x)\|\nabla (g_2-g_1)(x)\|_2.
	\end{equation*}

	Thus, in all cases, we conclude that
	\begin{equation*}
		\inf\{P(\epsilon) : H(\epsilon) \le 0, ~ \epsilon\in\Rd\} = (g_2-g_1)(x) - \frac{\beta r_2(x)^2}{2} - r_2(x)\|\nabla (g_2-g_1)(x)\|_2.
	\end{equation*}
	Substituting this result into the quadratic underestimation \eqref{eq: quadratic_underestimation}, we find that
	\begin{equation*}
		(g_2-g_1)(x+\delta) \ge (g_2-g_1)(x) - \frac{\beta r_2(x)^2}{2} - r_2(x)\|\nabla (g_2-g_1)(x)\|_2 = 0,
	\end{equation*}
	where the final equality comes from the definition of $r_2(x)$. Thus, we conclude that $f(x+\delta) = 2$.
\end{proof}
\end{comment}

Notice that $r_2(x) \ge 0$ for all $x\in \f^{-1}(\{2\})$ in Theorem \ref{thm: false_positive_robustness}. We may also provide a ``convex hull robustness'' guarantee for \cns, as Theorem \ref{thm: false_positive_robustness-convex_hull} below shows.

\begin{theoremrep}
	\label{thm: false_positive_robustness-convex_hull}
	
	Let $\f\in\F$ and let $X \subseteq \f^{-1}(\{2\}) = \{x\in\Rd : \f(x)=2\}$. Then $\f(x) = 2$ for all $x\in\conv(X)$.
\end{theoremrep}

\begin{proof}
	Let $x\in\conv(X)$, so that $x = \sum_{i=1}^N \theta_i x^{(i)}$ for some $x^{(1)},\dots,x^{(N)}\in X$ and some $\theta_1,\dots,\theta_N \ge 0$ satisfying $\sum_{i=1}^N \theta_i =  1$. Then, since $\g$ is convex, it holds that
	\begin{equation*}
		\g(x) = \g\left(\sum_{i=1}^N \theta_i x^{(i)}\right) \le \sum_{i=1}^N \theta_i \g(x^{(i)}) \le 0,
	\end{equation*}
	and therefore $\f(x) = 2$.
\end{proof}

The robustness granted by Theorem \ref{thm: false_positive_robustness-convex_hull} naturally corresponds to proving the absence of false positives in the case that \cs~associates to negatives and \cns~associates to positives. For example, when \cs~represents spam messages and \cns~represents nonspam, Theorem \ref{thm: false_positive_robustness-convex_hull} says that, given any set of nonspam messages, an adversary cannot fool the classifier into thinking a convex combination of the nonspam is spam. That is, the model class $\F$ in essence encodes a prior that convex combinations are not adversarial alterations of ``good'' data.

Notice that Theorem \ref{thm: false_positive_robustness-convex_hull} also grants a method to compute certified norm-balls, given that the norm balls can be written as the convex hull of a finite number of points. For example, given an input $x\in\Rd$ with $\f(x)=2$, if one would like to certify that $\f(x+\delta)=2$ for all $\delta\in\Rd$ such that $\|\delta\|_\infty \le \epsilon$ for some $\epsilon > 0$, Theorem \ref{thm: false_positive_robustness-convex_hull} shows that it suffices to show that $\f(x+\delta) = 2$ at every vertex $\delta$ of the $\|\cdot\|_\infty$-norm ball. Our characterization of $\f\in\F$ and its certified regions, as granted by Theorems \ref{prop: convex_decision_regions}, \ref{thm: false_negative_robustness}, \ref{thm: false_positive_robustness}, and \ref{thm: false_positive_robustness-convex_hull} is illustrated in Figure \ref{fig: regions}.

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.4\linewidth]{figs/regions.tikz}
	\caption{Illustration of decision regions (green and red) and certified regions (blue) for $\f\in\F$.}
        \label{fig: regions}
\end{figure}

Finally, we can also use $\beta$-smoothness to bound the suboptimality of the certified $\ell_2$-radius given in Theorem \ref{thm: false_negative_robustness}.

\begin{theoremrep}
	\label{thm: suboptimality_bound}
	Fix $\|\cdot\|=\|\cdot\|_*=\|\cdot\|_2$. Let $\f\in\F$, let $x\in \f^{-1}(\{1\}) = \{y\in\Rd : \f(y)=1\}$, let $r_1(x)\in\R_+$ be as in Theorem \ref{thm: false_negative_robustness}, and let $\hat{r}_1(x) \in \R_+$ be an arbitrary certified $\ell_2$-radius at $x$, meaning that $\f(x+\delta) = 1$ for all $\delta\in\Rd$ such that $\|\delta\|_2 < \hat{r}_1(x)$. If $\g$ is $\beta$-smooth with respect to $(\|\cdot\|_2,\|\cdot\|_2)$ and $r_1(x) < \frac{\| \nabla \g(x)\|_2}{ 2\beta}$, then it holds that
	\begin{equation*}
		0 \le \inf\{\|\delta\|_2 : \f(x+\delta) \ne 1, ~ \delta\in\Rd\} - \hat{r}_1(x) \le \sqrt{D(\mu^\star)} - \hat{r}_1(x),
	\end{equation*}
	where $D(\mu^\star) = -\frac{\|\nabla \g(x)\|_2^2{\mu^\star}^2}{2(2+\mu^\star\beta)} + \g(x)\mu^\star \ge 0$ and
	\begin{equation}
		\mu^\star = \frac{2}{\beta} \left(\frac{1}{\sqrt{1-\frac{2\beta r_1(x)}{\|\nabla \g(x)\|_2}} } - 1\right).
		\label{eq: suboptimality_bound_dual_variable}
	\end{equation}
\end{theoremrep}

\begin{proof}
	First, since $\hat{r}_1(x)$ is a certified $\ell_2$-radius at $x$, it holds that $\f(x+\delta) = 1$ for all $\delta\in\Rd$ such that $\|\delta\|_2 < \hat{r}_1(x)$, and therefore, if $\delta\in\Rd$ is such that $\f(x+\delta)\ne 1$, then necessarily it holds that $\|\delta\|_2 \ge \hat{r}_1(x)$, which proves the left-hand inequality.

	Next, suppose that $\g$ is $\beta$-smooth with respect to $(\|\cdot\|_2,\|\cdot\|_2)$. Then by Lemma 3.4 in \citet{bubeck2015convex}, it holds that
	\begin{equation*}
		\g(x+\delta) \le \g(x) + \nabla \g(x)^\top \delta + \frac{\beta}{2}\|\delta\|_2^2
	\end{equation*}
	for all $\delta\in\Rd$. Therefore, since $\f(x+\delta) \ne 1$ if and only if $\g(x+\delta) \le 0$, it holds that
	\begin{align*}
		\inf\{\|\delta\|_2 : \f(x+\delta) \ne 1, ~ \delta\in\Rd\} &= \inf\{\|\delta\|_2 : \g(x+\delta) \le 0, ~ \delta\in\Rd\} \\
		&\le \inf\{\|\delta\|_2 : \g(x) + \nabla \g(x)^\top \delta + \frac{\beta}{2}\|\delta\|_2^2 \le 0, ~ \delta\in\Rd\} \\
		&\eqqcolon p^\star.
	\end{align*}
	We now solve for the optimal value $p^\star$ in closed-form. Define $P = \frac{\beta}{2} I_d$, $q = \nabla \g(x)$, and $r = \g(x)$, and notice that
	\begin{equation*}
		(p^\star)^2 = \inf\{\delta^\top\delta : \delta^\top P\delta + q^\top\delta + r \le 0, ~ \delta\in\Rd\}
	\end{equation*}
	is a convex quadratically constrained quadratic program. The Lagrangian for the problem $(p^\star)^2$ is given by
	\begin{equation*}
		L(\delta,\mu) = \delta^\top \left(I_d + \mu P\right) \delta + \mu q^\top \delta + \mu r,
	\end{equation*}
	which is convex in $\delta$ for $\mu \ge 0$. The gradient with respect to $\delta$ is given by
	\begin{equation*}
		\nabla_\delta L(\delta,\mu) = 2(I_d+\mu P)\delta + \mu q,
	\end{equation*}
	which vanishes at
	\begin{equation*}
		\delta = -\frac{\mu}{2}(I_d+\mu P)^{-1}q.
	\end{equation*}
	This is well-defined for $\mu \ge 0$ since then $I_d+\mu P = \left(1+\frac{\mu\beta}{2}\right)I_d$ is positive definite and hence invertible. Therefore, the dual function $D\colon \R_+\to\R$ associated to the problem $(p^\star)^2$ is given by
	\begin{align*}
		D(\mu) &= \inf_{\delta\in\Rd} L(\delta,\mu) \\
		       &= \left(-\frac{\mu}{2}q^\top (I_d+\mu P)^{-1}\right)(I_d+\mu P)\left(-\frac{\mu}{2}(I_d+\mu P)^{-1} q\right) \\
		       &\quad+ \mu q^\top \left(-\frac{\mu}{2}(I_d+\mu P)^{-1} q\right) + \mu r \\
		       &= -\frac{\mu^2}{4} q^\top (I_d+\mu P)^{-1} q + \mu r.
	\end{align*}
	Since $P = \frac{\beta}{2}I_d$, this yields
	\begin{equation*}
		D(\mu) = -\frac{\mu^2}{2(2+\mu \beta)}q^\top q + \mu r.
	\end{equation*}
	The gradient of $D$ is given by
	\begin{align*}
		\nabla D(\mu) &= -\frac{\mu}{2+\mu\beta}q^\top q + \frac{\mu^2 \beta}{2(2+\mu\beta)^2}q^\top q + r \\
			      &= \frac{\beta q^\top q}{2} \left(\frac{\mu}{2+\mu\beta}\right)^2 - q^\top q \frac{\mu}{2+\mu\beta} + r.
	\end{align*}
	Since $r_1(x) < \frac{\|\nabla g(x)\|_2}{2\beta}$, it holds that $\frac{2\beta r}{q^\top q} < 1$, and therefore the equation $\nabla D(\mu) = 0$ has a unique solution $\mu^\star\in\R_+$ given by
	\begin{equation*}
		\mu^\star = \frac{2}{\beta}\left( \frac{1}{\sqrt{1-\frac{2\beta r}{q^\top q}} } - 1\right).
	\end{equation*}
	Notice that, by our definitions of $q$ and $r$, this $\mu^\star$ satisfies \eqref{eq: suboptimality_bound_dual_variable}. Evaluating $D$ at $\mu^\star$ yields
	\begin{equation*}
		D(\mu^\star) = \frac{\mu^\star}{2+\mu^\star \beta}\left(2r+\mu^\star\left(\beta r - \frac{q^\top q}{2}\right)\right),
	\end{equation*}
	which is nonnegative since $\mu^\star \ge 0$ and
	\begin{equation*}
		2r+\mu^\star\left(\beta r - \frac{q^\top q}{2}\right) = \frac{2}{\beta} \left(\frac{q^\top q}{2} - \sqrt{\left(\frac{q^\top q}{2}\right)^2 - \frac{q^\top q}{2} \beta r} \right) \ge 0.
	\end{equation*}
	This further shows that $D(0) = 0 \le D(\mu^\star)$, and therefore
	\begin{equation*}
		\sup_{\mu\in\R_+} D(\mu) = D(\mu^\star).
	\end{equation*}
	Now, taking $\delta = -K q \in\Rd$ with $K = \frac{1}{\beta}$ yields
	\begin{align*}
		\delta^\top P \delta + q^\top \delta + r &= K^2 q^\top \left(\frac{\beta}{2}I_d\right)q - K q^\top q + r \\
		&= \frac{1}{2\beta} q^\top q - \frac{1}{\beta} q^\top q + r \\
		&= -\frac{q^\top q}{2\beta} + r \\
		&<0,
	\end{align*}
	where the inequality comes from the fact that $\frac{2\beta r}{q^\top q} < 1$. Thus, the convex optimization $(p^\star)^2$ is strictly feasible, and therefore by Slater's condition it must be that strong duality holds. Hence,
	\begin{equation*}
		(p^\star)^2 = \sup_{\mu\in\R_+}D(\mu) = D(\mu^\star),
	\end{equation*}
	and therefore by definition of $p^\star$ this shows that
	\begin{equation*}
		\inf\{\|\delta\|_2 : \f(x+\delta) \ne 1, ~ \delta\in\Rd\} \le \sqrt{D(\mu^\star)},
	\end{equation*}
	which concludes the proof.
\end{proof}

\begin{remark}
	The hypothesis that $r_1(x) < \frac{\|\nabla \g(x)\|_2}{2\beta}$ in Theorem \ref{thm: suboptimality_bound} is key to utilizing $\beta$-smoothness to quantify the suboptimality of a certified radius $\hat{r}_1(x)$. Intuitively, this hypothesis ensures that the quadratic upper bound on $\g$ from $\beta$-smoothness is sufficiently tight so that it has zeros in $\Rd$. Without the existence of such zeros, the quadratic upper bound cannot be used to upper-bound the minimum adversarial radius $\inf\{\|\delta\|_2 : \f(x+\delta) \ne 1, ~ \delta\in\Rd\}$.
\end{remark}

We emphasize that the suboptimality bound in Theorem \ref{thm: suboptimality_bound} can be used to quantify how suboptimal an arbitrary certified radius $\hat{r}_1(x)$ is; one may want to use the certified radius $\hat{r}_1(x) = r_1(x)$ from Theorem \ref{thm: false_negative_robustness}, or alternatively, one may want to use the certified radius granted by randomized smoothing \citep{cohen2019certified} to characterize how suboptimal randomized smoothing is in the input-convex setting.\footnote{Notice that, for a binary input-convex base classifier $\f\in\F$, its associated smoothed classifier, defined by $\f^\sigma(x) = 1$ if $\g^\sigma(x) > 0$ and $\f^\sigma(x)=2$ if $\g^\sigma(x)\le 0$ with $\g^\sigma(x) = \expect_{\epsilon\sim \normal(0,\sigma^2 I_d)} \g(x+\epsilon)$, is also a binary input-convex classifier since expectation preserves convexity \citep[Section 3.2.1]{boyd2004convex}.}



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

